Dyck Words, Lattice Paths, and Abelian Borders

We use results on Dyck words and lattice paths to derive a formula for the exact number of binary words of a given length with a given minimal abelian border length, tightening a bound on that number from Christodoulakis et al. (Discrete Applied Mathematics, 2014). We also extend to any number of distinct abelian borders a result of Rampersad et al. (Developments in Language Theory, 2013) on the exact number of binary words of a given length with no abelian borders. Furthermore, we generalize these results to partial words.

==> eptcsdata.tex <==
\providecommand{\firstpage}{56}
\providecommand{\publicationstatus}{E. Csuhaj-Varj\'u, P. D\"om\"osi, Gy. Vaszil (Eds.): 15th International \\ Conference on Automata and Formal Languages (AFL 2017)\\
EPTCS 252, 2017, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.252.9}{10.4204/EPTCS.252.9}}
\pdfoutput=1

